Blind Identification of Fully Observed Linear Time-Varying Systems via Sparse Recovery

Discrete-time linear time-varying (LTV) systems form a powerful class of models to approximate complex dynamical systems with nonlinear dynamics for the purpose of analysis, design and control. Motivated by inference of spatio-temporal dynamics in breast cancer research, we propose a method to efficiently solve an identification problem for a specific class of discrete-time LTV systems, in which the states are fully observed and there is no access to system inputs. In addition, it is assumed that we do not know on which states the inputs act, which can change between time steps, and that the total number of inputs is sparse over all states and over time. The problem is formulated as a compressive sensing problem, which incorporates the effect of measurement noise and which has a solution with a partially sparse support. We derive sufficient conditions for the unique recovery of the system model and input values, which lead to practical conditions on the number of experiments and rank conditions on system outputs. Synthetic experiments analyze the method's sensitivity to noise for randomly generated models.

==> appendices.tex <==
\section{Sparse Recovery Theory}
\label{sec:AppendixSRT}
(NB: This Appendix is added to support the reviewer by providing theory with symbols similar as in the main manuscript. It can be omitted in the event of publication)
\subsection{Theory for Fully Sparse Support}
\label{sec:AppendixSRTa}
In the last decade, a rich body of new literature has formed to address the equivalence and exact recovery of compressed sensing problems, i.e. determining under what conditions the solution to \eqref{eq:CSP1} is equivalent and exactly recovers the solution to the NP-hard problem \eqref{eq:CSP0}. Here, we first address the results for noiseless case.
Exact recovery is generally assessed through inspection of the \emph{spark} property or, more practically, through the \emph{Mutual Coherence Condition} (MCC) of the sensing matrix $\Psi$.
The review paper \cite{bruckstein_sparse_2009} provides a solid overview of the theoretical principles developed for the canonical problem, in which the support of the solution vector is fully sparse. 
The following lemma enables the equivalence of solution between the non-convex compressed sensing problem and its convex relaxation.
Consider problem $P_1$ as introduced in \eqref{eq:CSP1}, with sensing matrix $\Psi \in \R^{m \times D}$.
\begin{definition}
The spark of a matrix $\Psi$ is the smallest number of columns of $\Psi$ that are linearly dependent.
\end{definition}
\begin{definition}
The mutual coherence of a matrix $\Psi$ is the largest absolute normalized inner product between different columns from $\Psi$. Denoting the $k$-th column in $\Psi$ by $p_k$, the mutual coherence is given by
\begin{equation}
\mu(\Psi) = \displaystyle \max_{1 \le k,j \le N , k \ne j} \dfrac{\left| p_k^{\top} p_j \right| }{\| p_k \|_2 \cdot \| p_j \|_2} 
\end{equation}
\end{definition}
Given these definitions, the following lemma adopted from \cite{bruckstein_sparse_2009} provides sufficient conditions for equivalence between the compressed sensing problem $P_0$ \eqref{eq:CSP0} and its convex relaxation $P_1$ \eqref{eq:CSP1}.
\begin{lemma} 
\label{lm:MCC}
(Equivalence - Spark and Mutual Coherence Condition)
For the system of linear equations $\Psi x = b$ ($\Psi \in \R^{D \times N}$ full-rank with $D < N$), if a solution $x$ exists obeying
\begin{equation}
\| x  \|_0 < \frac{1}{2}\left( 1 + \frac{1}{\mu(\Psi)}  \right) \le \frac{1}{2} \text{spark} (\Psi),
\end{equation}  
that solution is both the unique solution to the convex relaxation \eqref{eq:CSP1}, and the unique solution to the original NP-hard compressed sensing problem \eqref{eq:CSP0}.
\end{lemma}
The original proof was derived for the spark condition. The mutual coherence condition (MCC) provides a lower bound on the spark condition, for which a lemma is provided in \cite{bruckstein_sparse_2009}. The MCC is typically used as spark is expensive to compute. 
Notice that this result does not guarantee existence, but only provides the equivalence between solutions for the original problem \eqref{eq:CSP0} and its convex relaxation \eqref{eq:CSP1}.

Existence and uniqueness of the convex relaxation problem (our target problem) can be assessed through two different properties - the \emph{Null Space Property} (NSP), and the \emph{Restricted Isometry Property} (RIP) of the sensing matrix $\Psi$.
This theory was originally developed in \cite{donoho_optimally_2003} (NSP) and \cite{candes_restricted_2008} (RIP) for problems that have a solution with a fully sparse support. Here, we briefly state available theory that provides guarantees for extending these notions to scenarios with partial sparse support, which is critical to our problem formulation \eqref{eq:noiselessCS}. As assumed before, here we again need $\Psi_a$ to be full column rank.

Some notation: For sake of brevity, let $N = n k_f q + n^2 k_f$ be the dimension of our solution vector $[\pmb{u}^{\top} \ \pmb{a}^{\top} ]^{\top}$, and let $s$ denote its number of nonzero entries. Let $[N]$ represent the set of integers $\{ 1, 2, \hdots, N \}$, and $[N]^{(s)}$ the set of all subsets of $[N]$ of cardinality $s \le N$. Given $ \pmb{x} =  \in \R^N$ and $S \in [N]$, $x_S \in \R^N$ denotes a vector defined by $(\pmb{x}_S)_i = \pmb{x}_i , i \in S$ and $(\pmb{x}_S)_ i = 0 , i \notin S$. 
\begin{definition} (Null Space Property)
A matrix $\Psi \in \R^{D \times N}$ satisfies the Null Space Property (NSP) of order $s$ for  sparse recovery of size $N$ if, for every $\pmb{x} \in \R^{N}_{\backslash \{0\}}$ and every $S \in [N]^{(s)}$, we have
\begin{equation}
\| \pmb{x}_S \|_1 < \frac{1}{2} \| \pmb{x} \|_1
\end{equation}
\end{definition}
 
\begin{lemma} (NSP $\iff$ unique sparse recovery) The matrix $\Psi$ satisfies the Null Space Property of order $s$ if and only if, for every true $s$-sparse vector $\bar{\pmb{x}} = [\bar{\pmb{u}}^{\top} \ \bar{\pmb{a}}^{\top} ]^{\top} $, \eqref{eq:CSP1} with $\pmb{z} = \Psi \bar{\pmb{x}}$ has a unique solution given by $\pmb{x} = \bar{\pmb{x}}$. 
\label{thm:NSPunique}
\end{lemma}
 
\begin{definition} (Restricted Isometry Property)
A scalar $\delta_s > 0$ is the Restricted Isometry Property (RIP) constant of order $s$ of the matrix $\Psi \in \R^{D \times N}$ if it is the smallest positive real number such that
\begin{equation}
(1 - \delta_s) \| \pmb{x} \|_2^2 \le \| \Psi \pmb{x} \|_2^2 \le (1 + \delta_s) \| \pmb{x} \|_2^2
\end{equation}
for every $s$-sparse vector $\pmb{x}$.
\label{def:RIP}
\end{definition}

\begin{lemma} (RIP $\iff$ unique sparse recovery)
Let $\Psi \in \R^{D \times N}$ and $2s < D$. If $\delta_{2s} < \sqrt{2} - 1$, where $\delta_{2s}$ is the RIP constant of $\Psi$ of order $2s$, then the convex relaxation \eqref{eq:CSP1} with $\pmb{z} = \Psi \bar{\pmb{x}}$ has a unique solution given by $\pmb{x} = \bar{\pmb{x}}$, for every $s$-sparse vector $\bar{\pmb{x}}$.
\label{thm:RIPunique}
\end{lemma} 

In many realistic contexts, the measurement vector $y$ (as in \eqref{eq:CSP1}) contains noise and the signal $s$ is not sparse but \emph{compressible}. This means that many components are very small but not necessarily zero. Theoretical advances have generalized the Compressive Sensing framework to be robust to noise and recover compressible signals \cite{candes_restricted_2008}. 

\begin{lemma} 
\label{thm:compressible}
(Recovery of Compressible Signals) Assume that the matrix $\Psi \in \R^{m \times D}$ satisfies the RIP condition in Lemma \ref{thm:RIPunique} with RIP constant $\delta_{2s} < \sqrt{2} - 1$. For any true signal $\bar{x} \in \R^D$, let the noisy measurement be $y = \Psi \bar{x} + w$, with $\| w \|_2 \le \eta$. Let $x^*$ be a solution of 
\begin{equation}
P_2 \ : \ \displaystyle \min_{x \in \R^D} \| x \|_1 \quad \text{subject to} \quad \| \Psi x - y \|_2 \le \eta.
\end{equation}
Then it follows that the solution is close to the true signal as given by
\begin{equation}
\| x^* - \bar{x} \|_2 \le \alpha_1 \eta + \alpha_2 \dfrac{\sigma_s (\bar{x})_1}{\sqrt{s}},
\label{eq:stability1}
\end{equation}
with constants $\alpha_1,\alpha_2$ depending on RIP constant $\delta_{2s}$, and $\sigma_s (\bar{x})_1 = \min_{x : \| x \|_0 \le s} \| x - \bar{x} \|_1$.
\end{lemma}
The proof for this lemma can be found in \cite[Theorem 5.1]{bandeira_partial_2013}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Extension to Partially Sparse Support}
\label{sec:AppendixSRTb}
Several independent works have addressed the generalization to solutions for which part of the support of the solution $x$ is known \cite{bandeira_partial_2013,friedlander_recovering_2012,jacques_short_2010,vaswani_modified-cs:_2010}. The authors in \cite{bandeira_partial_2013} have focused their theory on the case where an a priori known part of the support of the solution is known to be dense, which relates to our problem formulation \eqref{eq:noiselessCS}, for which $\pmb{a}$ is generally a dense vector. 
We adopt two lemmas that outline these properties for partially sparse compressed sensing problems.

Let $r$ denote the number of entries in the dense part of our solution vector, i.e. $r = \text{dim}(\pmb{a}) = n^2 k_f$ (or $n^2$ in the LTI case).
\begin{definition} (Partial Null Space Property)
Our sensing matrix $\Psi = [\Psi_u \ | \ \Psi_a] \in \R^{D \times N}$ satisfies the Null Space Property (NSP) of order $s - r$ for partially sparse recovery of size $N - r$ with $r \le s$ if $\Psi_a$ is full column rank and for every $\pmb{u} \in \R^{N-r}_{\backslash \{0\}}$ such that $\Psi_u \pmb{u} \in \CMcal R (\Psi_a)$ and every $S \in [N - r]^{(s-r)}$, we have
\begin{equation}
\| (\pmb{u})_S \|_1 < \frac{1}{2} \| \pmb{u} \|_1
\end{equation}
\end{definition}
\begin{lemma} (Partial NSP $\iff$ uniqueness - adopted from \cite{bandeira_partial_2013})
The matrix $\Psi = [\Psi_u \ | \ \Psi_a] \in \R^{D \times N}$ satisfies the Null Space Property (NSP) of order $s - r$ for partial sparse recovery of size $N - r$ if and only if for every $\bar{\pmb{x}} = ( \bar{\pmb{x}}_1 , \bar{\pmb{x}}_2)$ such that $\bar{\pmb{x}}_1 \in \R^{N-r}$ is an $s-r$ sparse vector and $\bar{\pmb{x}}_2 \in \R^{r}$, problem \eqref{eq:noiselessCS} with $\pmb{z} = \Psi_u \pmb{u} +  \Psi_a \pmb{a}$ has a unique solution given by $(\pmb{u} , \pmb{a}) = (\bar{\pmb{x}}_1 ,\bar{\pmb{x}}_2)$.
\end{lemma} 
\begin{definition} (Partial RIP - adopted from \cite{bandeira_partial_2013})
$\delta_{s-r}^r > 0$ is the Partial Restricted Isometry Property Constant of order $s - r$ of the matrix $\Psi = [\Psi_u \ | \ \Psi_a] \in \R^{D \times N}$, for recovery of size $N - r$ with $r \le s$, if $\Psi_a$ is full column rank and $\delta_{s-r}^r$ is the RIP constant of order $s - r$ (see Definition \ref{def:RIP}) of the matrix $\CMcal P \Psi_u$, where $\CMcal P$ is given by \eqref{eq:proj}.
\end{definition}  

Notice that with $r = 0$ the Partial RIP reduces to the RIP of Definition \ref{def:RIP}. 
Combining Theorems \ref{thm:NSPunique} and \ref{thm:RIPunique}, one can show that, given a matrix $\Psi = [\Psi_u \ | \ \Psi_a] \in \R^{D \times N}$ with Partial RIP constant $\delta_{2(s-r)}^r$ of order $2(s-r)$ for recovery of size $N - r$, satisfying $\delta_{2(s-r)}^r < \sqrt{2} - 1$, $\CMcal P \Psi_u$ satisfies the NSP property of order $s - r$. 
Hence, given a true signal $\bar{\pmb{x}} = (\bar{\pmb{x}}_1,\bar{\pmb{x}}_2)$ such that $\bar{\pmb{x}}_1$ is $(s-r)$-sparse and $\bar{\pmb{x}}_2 \in \R^{r}$, $\bar{\pmb{x}}_1$ can be recovered by minimization of the $\ell_1$-norm of $\pmb{u}$ subject to $(\CMcal P \Psi_u)\pmb{u} = \CMcal P \Psi [\pmb{u}^{\top} \ \pmb{a}^{\top} ]^{\top}$ and, since $\Psi_a$ is assumed to be full column rank, $\pmb{a} = \bar{\pmb{x}}_2$ is uniquely determined by $\Psi_a \pmb{a} = \pmb{z} - \Psi_u \pmb{u} = \pmb{z} - \Psi_u \bar{\pmb{x}}_1$ \cite{bandeira_partial_2013}. In other words, this implies that $\Psi$ satisfies the NSP of order $s - r$ for partially sparse recovery of size $N - r$.

In short, we see that if we assume that $\Psi_a$ is full column rank and the sensing matrix $\Psi$ satisfies the NSP (Lemma \ref{thm:NSPunique}) or RIP (Lemma \ref{thm:RIPunique}) property, our problem \eqref{eq:noiselessCS} with partial sparse support will have a unique solution for any true signal $\bar{\pmb{x}}$.

Lastly, consider the result for retrieving a compressible signal in \eqref{thm:compressible}.
In our scenario the support of the true signal $\bar{x} = [\bar{x}_1^{\top} \ \bar{x}_2^{\top}]^{\top} $ is only partially sparse, i.e. $\bar{x}_2 \in \R^r$ is a dense vector. The following lemma extends Lemma \ref{thm:compressible} to this scenario.
\begin{lemma} (Recovery of Compressible Signals with Partially Sparse Support)
\label{thm:partialsparse_stability}
Since $\CMcal P$, as in \eqref{eq:proj}, is a projection matrix, we have that $\| \CMcal P \Psi_1 \bar{x}_1 - \CMcal P y \|_2 = \| \CMcal P \Psi \bar{x} - \CMcal P y \|_2 \le \| \Psi \bar{x} - y \|_2 \le \eta$, and the solution $x^*$ of 
\begin{equation}
P_3 \ : \ \displaystyle \min_{x_1 \in \R^{D-r}} \| x_1 \|_1 \quad \text{subject to} \quad \| \CMcal P \Psi_1 x_1 - \CMcal P y \|_2 \le \eta
\end{equation}
satisfies
\begin{equation}
\| x_1^* - \bar{x}_1 \|_2 \le \beta_1 \eta + \beta_2 \dfrac{\sigma_{s-r} (\bar{x}_1)_1}{\sqrt{s-r}},
\label{eq:stability2}
\end{equation}
where $\beta_1,\beta_2$ now depend on the RIP constant. $x^*_2$ is determined by $\Psi_2 x^*_2 = y - \Psi_1 x^*_1$, and obeys:
\begin{equation}
\| x_2^* - \bar{x}_2 \|_2 \le C_2 \left( 2 \eta + C_1 \left( \beta_1 \eta + \beta_2 \dfrac{\sigma_{s-r} (\bar{x}_1)_1}{\sqrt{s-r}} \right) \right),
\label{eq:stability_a}
\end{equation}
where $C_1 = \| \Psi_1 \|_2$ and $C_2 = \| \Psi^{\dagger}_2 \|_2$, with $\Psi^{\dagger}_2 = (\Psi^{\top}_2 \Psi_2)^{-1}\Psi^{\top}_2$.
\end{lemma}
The proof for this lemma can be found in \cite[Theorem 5.2]{bandeira_partial_2013}.




==> background.tex <==
\section{Background on Sparse Recovery}
\label{sec:background}

This work has been primarily motivated by advances in Sparse Recovery Theory \cite{candes_compressive_2006,donoho_for_2006}. The formulation of our problem will entail visiting a canonical problem in this field: Compressive Sensing (CS).
In the last decade, CS has developed as a significant area of signal processing that has challenged basic assumptions on the amount of data (sampling rate or number of data points) needed to recover a signal. 
Consider the measurement equation
\begin{equation}
y = \Psi x + w, 
\label{eq:measeq}
\end{equation}
where $y \in \R^m, x \in \R^D$, and $\| w \|_2 \le \eta$ is a bounded noise signal. 
In general, $m<D$ yields an underdetermined system of equations, with an infinite number solutions. It turns out that if the \emph{sensing matrix} $\Psi$ adheres to certain conditions, $x$ can be retrieved exactly from far fewer measurements (i.e. $m \ll D$) than asserted by the Nyquist sampling theorem \cite{bruckstein_sparse_2009}.
The sparsest solution to the underdetermined system of equations $y = \Psi x$ can be found by solving:
\begin{equation}
\displaystyle \min_{x \in \R^D} \| x \|_0 \quad \text{subject to} \quad y = \Psi x.
\label{eq:CSP0}
\end{equation}
The following lemma \cite[Lemma 2.1]{donoho_for_2006} provides a sufficient condition that the solution to \eqref{eq:CSP0} is unique:
\begin{lemma}
If the sparsest solution to \eqref{eq:CSP0} has $\| x \|_0 = s$ and $D \ge 2s$ and all subsets of $2s$ columns of $\Psi$ are full rank, then this solution is unique.
\label{thm:uniqueness}
\end{lemma}

In general, \eqref{eq:CSP0} is a NP-hard optimization problem that is both combinatorial and non-convex, and hence impractical to solve. 
In contrast, the \emph{Basis Pursuit} method \cite{chen_atomic_2001} solves the convex relaxation of \eqref{eq:CSP0} efficiently:
\begin{equation}
\displaystyle \min_{x \in \R^D} \| x \|_1 \quad \text{subject to} \quad y = \Psi x.
\label{eq:CSP1}
\end{equation}
Consider the following two definitions.
\begin{definition}
The spark of a matrix $\Psi$ is the smallest number of columns of $\Psi$ that are linearly dependent.
\end{definition}
\begin{definition}
The mutual coherence of a matrix $\Psi$ is the largest absolute normalized inner product between different columns from $\Psi$. Denoting the $k$-th column in $\Psi$ by $p_k$, the mutual coherence is given by
\begin{equation}
\mu(\Psi) = \displaystyle \max_{k \ne j} \dfrac{\left| p_k^{\top} p_j \right| }{\| p_k \|_2 \cdot \| p_j \|_2} 
\end{equation}
\end{definition}
Given these definitions, the following lemma adopted from \cite{bruckstein_sparse_2009} provides sufficient conditions for equivalence between the compressed sensing problem \eqref{eq:CSP0} and its convex relaxation \eqref{eq:CSP1}.
\begin{lemma} 
\label{lm:equiv}
(Equivalence - Spark and Mutual Coherence Condition)
For the system of linear equations $\Psi x = y$ ($\Psi \in \R^{m \times D}$ full-rank with $m < D$), if a solution $x$ exists obeying
\begin{equation}
\| x  \|_0 < \frac{1}{2}\left( 1 + \frac{1}{\mu(\Psi)}  \right) \le \frac{1}{2} \text{spark} (\Psi),
\end{equation}  
that solution is both the unique solution to the convex relaxation \eqref{eq:CSP1}, and the unique solution to the original NP-hard compressive sensing problem \eqref{eq:CSP0}.
\end{lemma}
The original proof was derived for the spark condition. The mutual coherence condition (MCC) provides a lower bound on the spark condition, for which a lemma is provided in \cite{bruckstein_sparse_2009}. The MCC is typically used as spark is expensive to compute. 
Notice that this result does not guarantee existence, but only provides the equivalence between solutions for the original problem \eqref{eq:CSP0} and its convex relaxation \eqref{eq:CSP1}.
%It has been shown that for sufficiently large $m$ and a sufficiently \emph{incoherent} sensing matrix $\Psi$, the solutions to \eqref{eq:CSP1} and \eqref{eq:CSP0} are exact \cite{candes_sparsity_2007}.
%Incoherence of a matrix is defined as 
%\begin{equation}
%\mu(\Psi) \triangleq \max_{i,j} \frac{| \psi_i^{\top} \psi_j |}{\| \psi_i \|  \| \psi_j \|}
%\end{equation}
%which can be interpreted as the maximum angle between two arbitrary columns of $\Psi$, or in other words how orthogonal its columns are.

In the presence of measurement noise, it can be shown that the optimal sparse solution $x^*$ to \eqref{eq:CSP1} is \emph{compressible}, that is many of its entries are very close to zero. The canonical problem that allows for recovering a compressible signal looks as follows:
\begin{equation}
\displaystyle \min_{x \in \R^D} \| x \|_1 \quad \text{subject to} \quad \| y - \Psi x \| \le \eta.
\label{eq:CSP2}
\end{equation}
where $\eta$ is an \emph{a priori} known bound on the measurement noise $w$ in \eqref{eq:measeq}.
Many theoretical results have followed in recent years to assess under what conditions \eqref{eq:CSP2} recovers the exact solution within tight bounds, mainly centering around the Null Space Property and the Restricted Isometry Property.
Let $s$ denote the number of nonzero entries of solution vector $x$. 
\begin{definition} (Null Space Property)
A matrix $\Psi \in \R^{m \times D}$ satisfies the Null Space Property (NSP) of order $s$ for sparse recovery of size $D$ if, for every $x$ in the null space of $\Psi{\backslash \{0\}}$ and every $S \in [D]^{(s)}$, we have
\begin{equation}
\| x_S \|_1 < \frac{1}{2} \| x \|_1
\end{equation}
\end{definition}
 
\begin{lemma} (NSP $\iff$ unique sparse recovery \cite{donoho_optimally_2003}) The matrix $\Psi$ satisfies the Null Space Property of order $s$ if and only if, for every true $s$-sparse vector $\bar{x}$, \eqref{eq:CSP1} with $y = \Psi \bar{x}$ has a unique solution given by $x = \bar{x}$. 
\label{thm:NSPunique2}
\end{lemma}
 
\begin{definition} (Restricted Isometry Property)
A scalar $\delta_s > 0$ is the Restricted Isometry Property (RIP) constant of order $s$ of the matrix $\Psi \in \R^{m \times D}$ if it is the smallest positive real number such that
\begin{equation}
(1 - \delta_s) \| x \|_2^2 \le \| \Psi x \|_2^2 \le (1 + \delta_s) \| x \|_2^2
\end{equation}
for every $s$-sparse vector $x$.
\label{def:RIP}
\end{definition}

\begin{lemma} (RIP $\iff$ unique sparse recovery \cite{candes_restricted_2008})
Let $\Psi \in \R^{m \times D}$ and $2s < D$. If $\delta_{2s} < \sqrt{2} - 1$, where $\delta_{2s}$ is the RIP constant of $\Psi$ of order $2s$, then the convex relaxation \eqref{eq:CSP1} with $y = \Psi \bar{x}$ has a unique solution given by $x = \bar{x}$, for every $s$-sparse vector $\bar{x}$.
\label{thm:RIPunique2}
\end{lemma} 

In Section \ref{sec:analysis} we will utilize and extend these results to address research questions relevant for the system identification and input retrieval problem defined in the next section.

%\subsection{Brief Overview of Sparse Recovery Theory Results}
%A natural first question to ask is under what conditions the solution to the convex surrogate problem \eqref{eq:CSP1} exactly recovers a \emph{particular solution} to the original problem \eqref{eq:CSP0}.  Exact recovery is generally assessed through inspection of the \emph{spark} property or, more practically, through the \emph{Mutual Coherence Condition} (MCC) of the sensing matrix $\Psi$.
%The review paper \cite{bruckstein_sparse_2009} provides a solid overview of the theoretical principles developed for the canonical problem, which provides sufficient conditions for exact recovery if the sparsity of the particular solution obeys an inequality that is a function of the spark or MCC of the sensing matrix. 
%A second question is for what conditions on the sensing matrix $\Psi$ \emph{any solution} $x$ of sparsity degree $s$ can be retrieved exactly and uniquely. Two sufficient conditions were discovered, namely the \emph{Null Space Property} (NSP), and the \emph{Restricted Isometry Property} (RIP) of the sensing matrix $\Psi$, originally developed in \cite{donoho_optimally_2003} (NSP) and \cite{candes_restricted_2008} (RIP) respectively. 
%The last question we should consider is under what conditions we can successfully recover a solution with measurements that are subject to noise, which is a given in many realistic contexts. As a result, the measurement vector $y$ (as in \eqref{eq:CSP1}) contains noise and the signal $x$ is not sparse but \emph{compressible}. This means that many components are very small but not necessarily zero. Theoretical advances have generalized the Compressive Sensing framework to be robust to noise and recover compressible signals. 
%Along with the development of the RIP property, a condition was developed in the case of bounded noise, which bounds the distance between the solution and the true value \cite{candes_restricted_2008}.
%
%Appendix \ref{sec:AppendixSRTa} succinctly covers the above notions, and Appendix \ref{sec:AppendixSRTb} then refers to recently developed extensions that provides guarantees for  problems that have a solution with a partially sparse support, which is critical to our problem formulation (\ref{eq:noisyCS}-\ref{eq:noiselessCS}). 
%Several independent works have addressed the generalization to solutions for which part of the support of the solution $x$ is known \cite{bandeira_partial_2013,friedlander_recovering_2012,jacques_short_2010,vaswani_modified-cs:_2010}. The authors in \cite{bandeira_partial_2013} have focused their theory on the case where an a priori known part of the support of the solution is known to be dense, which relates to our problem formulation \eqref{eq:noiselessCS}, for which $\pmb{a}$ is generally a dense vector unless the system's network or dynamics are sparsely connected. 
%Via a projection procedure our problem can be formed into the canonical problem. This helps extending the canonical theoretical results.
%\todo[inline]{What do we think of this overview? Is it clear? And can we put all this material in the Appendix?}



